A systematic literature review on counterexample explanation

Context: Safety is of paramount importance for cyber-physical systems in domains such as automotive, robotics, and avionics. Formal methods such as model checking are one way to ensure the safety of cyber-physical systems. However, adoption of formal methods in industry is hindered by usability issues, particularly the difficulty of understanding model checking results. Objective: We want to provide an overview of the state of the art for counterexample explanation by investigating the contexts, techniques, and evaluation of research approaches in this field. This overview shall provide an understanding of current and guide future research. Method: To provide this overview, we conducted a systematic literature review. The survey comprises 116 publications that address counterexample explanations for model checking. Results: Most primary studies provide counterexample explanations graphically or as traces, minimize counterexamples to reduce complexity, localize errors in the models expressed in the input formats of model checkers, support linear temporal logic or computation tree logic specifications, and use model checkers of the Symbolic Model Verifier family. Several studies evaluate their approaches in safety-critical domains with industrial applications. Conclusion: We notably see a lack of research on counterexample explanation that targets probabilistic and real-time systems, leverages the explanations to domain-specific models, and evaluates approaches in user studies. We conclude by discussing the adequacy of different types of explanations for users with varying domain and formal methods expertise, showing the need to support laypersons in understanding model checking results to increase adoption of formal methods in industry.

==> tex/RQ.tex <==
\section{Research Questions}
\label{sec:RQ}

The main motive of this survey is to address the general question: \textit{What is the state of the art for explaining counterexamples generated by model checkers?}
We argue that counterexample explanation is a key for a broader adoption of model checking because it allows the use of model checkers without necessarily having to understand their inner workings. Moreover, it promises to make the model checking result actionable for engineers by supporting them to understand and localize the fault in the system design.

To answer the general question with our survey, we refined it to
eight
specific research questions.
\fig{overview} positions each of these research questions in our conceptual overview of model checking and counterexample explanation. We present quantitative analysis results wherever reasonable and provide additional qualitative results and highlight exemplary publications.

% Representation
\rsqparagraph{1}{How are counterexamples represented and what are the effects of the counterexample representation on its interpretation?}
With this question we want to investigate how counterexamples and their explanations are presented to the engineer, \ie which style of representation is used and what effects do these have on the interpretation of counterexamples by engineers. \lars{my initial impression was that this can be cut or merged with other RQ}

% System Description
\rsqparagraph{2}{For which systems descriptions and input domains are counterexample explanation approaches available? What is the influence of the input domain on the explanation?}
What are the system descriptions and input domains used in counterexample explanation? Are they usually the same as the output domain and how does this impact does this have on representing and explaining counterexamples?

% System Specification
\rsqparagraph{3}{How are system specifications expressed and what properties do they cover?}\\

% Frameworks and tools
\rsqparagraph{4}{Which frameworks and verification tools are developed and used to represent and explain counterexamples?}\\
Which frameworks are developed or used to represent and explain counterexamples?
What impact does the used verification tool and framework have on representing and explaining counterexamples?

% Processing
\rsqparagraph{5}{How are counterexamples further processed and what effect does it have on interpreting the counterexample?}\\
Answering this question provides a summary of the effects of the processed counterexample on the interpretation of the counterexample. In \fig{overview}, this question addresses the \concept{processed counterexample} and how it is created from the counterexample (\step{4}), as well as how both of them impact the interpretation of the counterexample by engineers (\step{6}).

% Enriching
\rsqparagraph{6}{What kind of additional information is provided for enriching the counterexample representation?}\\
This question investigates additional information that is provided along with this counterexample to improve the counterexample representation for debugging the system and locating errors.

% Evaluation
\rsqparagraph{7}{How are counterexample explanation approaches evaluated?}\\
This question provides insights into how counterexample explanation approaches are evaluated, \ie the evaluation methods, domains and applications, as well as the evaluated aspects.

\paragraph{Summary}
Considering \fig{overview} in which all of the research questions are positioned in a conceptual overview of model checking and counterexample explanation, we observe that the research questions tackle all relevant elements. Therefore, we think that our survey can provide a comprehensive overview of the state of the art in counterexample explanation.


==> tex/Synopsis.tex <==
\section{Synopsis}

==> tex/rsq-properties-kicked-out.tex <==
\subsubsection{\rsq{3}: Properties, verification tools, and input domains}
\label{sec:analysis:rsq3}

%\arut{need to add citation and abbreviation for logics and model checker. i will do it later}
As shown in \fig{overview}, the verification tool verifies whether the provided requirement is satisfied by the given system. 
This research questions investigates which specification properties are used, which input domains are used pre-dominantly, and which tools are used for verification.

\subsubsection{Specification properties}

\begin{figure}
	\centering
	\includegraphics[scale=.75]{fig/rsq3prop.png}
	\caption{Types of specification properties}
	\label{fig:rsq3prop}
\end{figure}

Temporal logics can be specified as \emph{safety} and \emph{liveness} property. Safety properties assert that something bad never happens, while liveness properties assert that something good will eventually happen~\cite{Sistla94}. A counterexample to a liveness property in a finite system is lasso-shaped, which consists of a prefix that leads to a loop. For safety properties, a counterexample is finite in length~\cite{BiereAS02}. As shown in \fig{rsq3prop}, most of the surveyed publications address safety properties, or safety and liveness at the same time~\cite{EdelkampLL01,EdelkampLL04,SchuppanB05}.

\subsubsection{Key-Message}

Looking on \fig{rsq3mc} and \fig{rsq3spec}, the quantitative results for verification tools and temporal logics are influenced by one another. This is because certain logics can be recognized only by some verification tools and the same is true the other way around. For example, in \fig{rsq3spec}, we see \gls{LTL} is the most used logic. Further, looking on \fig{rsq3mc}, some of the most used verification tools are \gls{NuSMV}/\gls{SMV}, \gls{SPIN} and Maude which can realize \gls{LTL} logics.

In our survey, we found a considerable number of publications for verifying probabilistic specification but there is only one project that deals with counterexample interpretation of real-time specifications: the work by Gerking \etal~\cite{GerkingSDH15} using UPPAAL as verification tool. 

As shown in \fig{rsq3prop}, roughly half of the surveyed work deals with a combination of both safety and liveness properties. While almost every publication is found to focus on safety properties, only 11\% are found to address the liveness property.


==> tex/rsq_methods.tex <==
\subsection{\rsq{5}: Methods/Techniques used to process or represent counterexamples}
\label{sec:analysis:method}

Technically, the processed counterexamples and counterexample representations play a huge role in the counterexample interpretation and explanation (ref. \fig{overview}).\arne{"technically" they play a huge role? what is this supposed to mean?} Various methods and techniques from the literature for the counterexample interpretations are discussed as follows. 
Publications related to this question are listed in \tab{methods}.

\subsubsection{Search methods}
\label{sec:analysis:method:search}

Most of the search methods\arne{you didn't introduce the term, yet.} that are found from the literature are used for minimizing the counterexample. The work from Tan \etal~\cite{TanACZL04} reduces the size of the counterexample by using a \emph{heuristic-guided search strategy}. It is used to associate the estimated metric with every node.\arne{The reader doesn't know anything about a metric or node here.} Then during search, this metric is used to discriminate among the nodes.\arne{no chance to understand what you are talking about without reading the cited paper. I think you need to introduce what "search methods" are in this context (something with a graph probably) and while doing so (very shortly), introduce what nodes and metrics have to do with it.}

Edelkamp \etal~\cite{EdelkampLL01,EdelkampLL04} present the \emph{A$\ast$ directed search algorithms} and propose heuristics for the search of safety property violations. It accelerates the search in the direction of a specified failure situation, with an improved \emph{nested \gls{DFS}} algorithm that exploits the structure of \emph{Promela Never-Claims}. Aljazzar and Leue~\cite{AljazzarL08} visualize the state-space of Markov chain as a directed graph where states are represented by node icons and transition are represented by lines. To determine the shortest path in a directed graph, Aljazzar and Leue applied A$\ast$ algorithm where all the edges from the given directed graph are explored and inserted into a graph structure called \emph{path graph}. 

Gastin and Moro~\cite{GastinM07} propose a polynomial-time algorithm to compute a counterexample of minimal size for \gls{SPIN} that uses forward edges and consumes less memory than SPIN, while trying to reduce the size of counterexamples. It is based on \emph{\gls{BFS}} which is driven by the priority queue.
Similarly, Gastin \etal~\cite{GastinMZ04} use \emph{\gls{DFS}} that can actually display the sequence of counterexamples, that are decreasing in length. They are found during its execution and can be stopped at any time. 
Furthermore, model checker Maude~\cite{NguyenO17} is equipped with the search command where the command exhaustively traverses the reachable states in breadth-first manner to generate the shortest counterexample.

Leitner-Fischer and Leue~\cite{Leitner-FischerL14} integrate \gls{DFS} and \gls{BFS} for the causality checking, where a bad or good execution is detected by the search algorithm, and then added to a special data structure that is used to compute the causality relationships.
The work from Hansen and Kervinen~\cite{HansenK06} perform three different searches by using \gls{BFS}: first one to find the depth of each state, second search to find the shortest path from a Buchi state to all other states, and the third one to find the shortest path from other states to the Buchi state. While the first two searches are made using a regular \gls{BFS}, whereas the last one is carried out using a backward search that explores the edges backwards. 

The algorithm by Groce and Visser~\cite{GroceV03} generates a subset of \emph{negatives} - executions that reach a particular error state, and a set of potential \emph{positives} - any execution that do not end up in the error state, and uses a model checker to explore backward from the original counterexample. The algorithm is depth-first, but it can be integrated into both breadth-first and heuristic-based model checking algorithms.
A directed explicit state-space search strategy called \emph{\gls{XBF}} explores the state transition graph of \glspl{CTMC} and \glspl{DTMC}. It incrementally determines a sub-graph of the state transition graph, which covers the most probable diagnostic paths~\cite{AljazzarL10}. \gls{XBF} based algorithms are guided by heuristics to amplify the power of search, in-terms of computational efforts and counterexample quality.
\arne{this subsection is a very detailed overview ith lots of interesting references. however, it does not yet have a clear structure, e.g., clustering similar approaches}

\subsubsection{Other approaches}
\label{sec:analysis:method:other}

\gls{BFL} is the most effective counterexample minimization algorithm~\cite{ShenQL05-1,ShenQL05-2}. It performs refutation analysis of counterexample variables, \ie to extract the set of variables that are irrelevant to the counterexample. Thus, multiple variables can be eliminated with only one call to the \gls{SAT} solver. The algorithm proposed by Weitl and Nakajima~\cite{WeitlN10} generates the counterexample incrementally for ALCCTL, where a coarse counterexample is generated initially and subsequently refined to the desired level.\arne{I don't understand how elimination of variables has to do with refinement (of what?).} Further, the refinement of the counterexample is the user's choice; it is performed interactively in a step-by-step manner based on the error scenario. 

The approach presented by Ball \etal~\cite{BallNR03} generates multiple error traces by making use of the existing correct traces in order to localize the error cause. This is similar to SLAM\cite{glossray? citation?} that verifies C programs and localizes the errors in device drivers. The algorithm performs the following functions in the program: highlighting each error location, introducing halt statements and re-running the model checker to produce additional error traces.

Leue and Befrouei~\cite{LeueB12} use \gls{SPIN} for detection of deadlock in a concurrent system, where a set of counterexamples is generated as a bad dataset\arne{are they using this term in the publciation?} and an additional possible good dataset is generated that does not violate the property. By comparing the bad dataset with a good dataset, sequence of actions are extracted to locate the cause of occurrence of deadlock. Two different approaches are used by Kumar \etal~\cite{KumarKV05} for error explanation. The first approach is to compute the minimal change in a system, to eliminate the error cause for counterexample generation. In the second approach, the correct trace of the system that is close to the counterexample is computed.

\subsubsection{Key-Message}
\label{sec:analysis:method:conclusion}

Counterexample minimization is found to be the most used counterexample processing. Search methods found from the literature are mostly supported for minimizing a counterexample by using the model checkers like \gls{SPIN} and Maude.\arne{I don't understand the statement (language). Do you want to say that most of the search-based approaches use Spin and maude?}

Model transformation is another method used for minimizing counterexamples. These approaches rely on domain-specific input from the user and transform it to formal notations supported for verification. Further, the counterexample generated during verification is translated back to the user given input.
This hides the complexity of using formal logic and thus, the approach performs both the model abstraction and the counterexample representation or visualization.

